Equivariant Deep Learning of Mixed-Integer Optimal Control Solutions for Vehicle Decision Making and Motion Planning

Mixed-integer quadratic programs (MIQPs) are a versatile way of formulating vehicle decision making and motion planning problems, where the prediction model is a hybrid dynamical system that involves both discrete and continuous decision variables. However, even the most advanced MIQP solvers can hardly account for the challenging requirements of automotive embedded platforms. Thus, we use machine learning to simplify and hence speed up optimization. Our work builds on recent ideas for solving MIQPs in real-time by training a neural network to predict the optimal values of integer variables and solving the remaining problem by online quadratic programming. Specifically, we propose a recurrent permutation equivariant deep set that is particularly suited for imitating MIQPs that involve many obstacles, which is often the major source of computational burden in motion planning problems. Our framework comprises also a feasibility projector that corrects infeasible predictions of integer variables and considerably increases the likelihood of computing a collision-free trajectory. We evaluate the performance, safety and real-time feasibility of decision-making for autonomous driving using the proposed approach on realistic multi-lane traffic scenarios with interactive agents in SUMO simulations.

==> variable_table.tex <==
\begin{table}
	\centering
	\ra{1.2}
	\begin{tabular}{@{}ccl@{}}
		\addlinespace
		\toprule
		Symbol & Dimension & Description\\
		\midrule
		$\dimKin $ &$\mathbb{Z}$& 				Number of kinematic vehicle states \\
		$\dimPm $ &$\mathbb{Z}$& 	Number of point mass states \\
		$\dimSim $ &$\mathbb{Z}$& 	Number of simulator model states\\
		$\dimContr $ &$\mathbb{Z}$&  				Number of model inputs\\
		$\dimObs $ &$\mathbb{Z}$& 	Number of obstacles\\
		$\dimHor $ &$\mathbb{Z}$& 	Number of discretization steps\\
		$\dimBin $ &$\mathbb{Z}$& 	Number of binary variables\\
		$\dimBinL $ &$\mathbb{Z}$& 	Number of unstructured binary variables\\
		$\dimBinY $ &$\mathbb{Z}$& 	Number of equivariant binary variables\\
		$\dimSet $ &$\mathbb{Z}$& 	Number of equivariant set elements\\
		$\dimFeatEq $ &$\mathbb{Z}$& 	Number of equivariant features\\
		$\dimFeatUs $ &$\mathbb{Z}$& 	Number of unstructured features\\
		$M $ &$\mathbb{Z}$& 	"large number" used in "big-M" notation\\
		\midrule
		$\xPm $ & 		$\mathbb{R}^{\dimPm}$ & Point-mass model state\\
		$\xExp $ & 		$\mathbb{R}^{\dimPm}$ & Expert state\\
		$\xNN{i} $ &	$\mathbb{R}^{\dimPm}$ & Predicted state of $i$-th network\\
		$\xCor $ &		$\mathbb{R}^{\dimKin}$& Corrected state\\
		$\xMpc $ &		$\mathbb{R}^{\dimKin}$& MPC state \\
		$\xSim $ &		$\mathbb{R}^{\dimSim}$& Simulator state\\
		\midrule
		$\xOpp $ &$\mathbb{R}^{\dimKin}$& Obstacle states\\
		$\bin $ & $\mathbb{B}^{\dimBin}$ & Binary variables \\
		$\binY_j $ & $\mathbb{B}^{\dimBinY}$ & Binary equivariant variables \\
		$\binL $ & $\mathbb{B}^{\dimBinL}$ & Binary unstructured variables \\
		$\Bin $ & $\mathbb{B}^{\dimBin \times \dimHor}$ & Binary variable trajectory \\
		$\BinY $ & $\mathbb{B}^{\dimBinY \times \dimHor}$ & Binary eq. variable trajectory \\
		$\BinL $ & $\mathbb{B}^{\dimBinL \times \dimHor}$ & Binary unstr. variable trajectory \\
		\midrule
		$\setCar $ && Occupied space of vehicle\\
		$\setSafe $ && Inflated space of vehicle\\
		$\setOut $ && Rectangular over-approx. of $\setSafe$\\
		$\setFreeSafe $ && Free space related to $\setSafe$\\
		$\setFreeOut $ && Free space related to $\setOut$ \\
		\midrule
		$\EqSet $ && Permutation equivariant set\\
		$\eqFeat_{j} $ & $\mathbb{R}^{\dimFeatEq}$ & Equivariant feature of set element $j$\\
		$\usFeat $ &$\mathbb{R}^{\dimFeatUs}$& Unstructured features\\
		$\eqLab_{j,i} $ &$\mathbb{B}^{\dimBinY}$& Equivariant true labels at time step $i$\\
		$\usLab_{i} $ &$\mathbb{B}^{\dimBinL}$& Unstructured true labels  at time step $i$\\
		\midrule
		$\acc $ && Accuracy\\
		$\feas $ && Feasibility\\
		$\tcomp $ && Computation time\\
		$\costRatio $ && Cost ratio \\
		$\cost $ && Cost, Optimization objective\\		
		\bottomrule
		\vspace{0.5px}
	\end{tabular}
	\caption{Symbols and dimensions}
	\label{table:symbols}
\end{table}
